A Neural JKO Scheme for Hellinger-Kantorovich Gradient Flows via Monge-Growth Pairs

We develop a mesh-free neural JKO scheme for advection-reaction-diffusion equations with a gradient-flow structure in the Hellinger-Kantorovich (HK) geometry of unbalanced optimal transport. Each update is parametrized by a spatial map and a mass-changing factor, allowing spatial redistribution and local mass creation or loss to be treated jointly within a single variational step. Their cone action bounds the squared HK distance from above, yielding a sufficient condition for discrete energy dissipation through comparison with the identity pair. Minimizing the pair objective over all admissible pairs recovers the exact JKO minimum when the source and a minimizer have positive densities. We establish existence and mass bounds for JKO minimizers and, under additional assumptions, obtain positivity and regularity together with a discrete Euler-Lagrange equation and a metric-dissipation identity. The self-consistent chemical potential is then nonincreasing along an optimal map. There exist parametric pairs whose endpoint densities and objective values converge to those of an exact JKO minimizer, provided a regular-pair approximation hypothesis holds. Finally, we show that a primal-dual gap controls objective suboptimality and, for Boltzmann entropy, the $L^1$ density error, assuming exact-step regularity, positive-semidefinite interactions, and global dual feasibility. Numerical experiments examine pointwise agreement with the PDE, energy dissipation, and the roles of transport, reaction, and fully implicit interactions.

==> generated/density_family_table.tex <==
\begin{tabular}{@{}lcll@{}}
\toprule
Experiment & $d$ & pair-training rule & density family \\
\midrule
Entropy--potential & 1 & Gauss--Legendre $257$ & mixed-activation FCNN \\
Entropy--potential & 2 & Gauss--Legendre $4225$ & mixed-activation FCNN \\
$\HK$ entropy flow & 2 & -- & -- \\
$\HK$ entropy flow & 8 & importance draws $2048$ & mixed-activation FCNN \\
Fokker--Planck type & 2 & Gauss--Legendre $1089$ & mixed-activation FCNN \\
Fokker--Planck type & 4 & -- & -- \\
Implicit interaction & 2 & periodic grid $961$ & mixed-activation FCNN \\
\bottomrule
\end{tabular}


==> generated/diagnostics_table.tex <==
\begin{tabular}{@{}lccccccc@{}}
\toprule
Experiment & $d$ & rel. $L^2$ & $\max_k$ rel. $L^2$ & $\overline{\mathcal A^{\rm tr}/\mathcal A}$ & reference & $\min J_T$ & $\sup\|D\delta\|$ \\
\midrule
Entropy--potential & 1 & 2.006e-05 & 9.819e-03 & 0.150 & 0.145 & 0.981 & 0.539 \\
Entropy--potential & 2 & 5.319e-04 & 0.016 & 0.105 & 0.102 & 0.969 & 0.644 \\
$\HK$ entropy flow & 2 & -- & -- & -- & -- & -- & -- \\
$\HK$ entropy flow & 8 & 8.029e-03 & 8.029e-03 & 0.069 & 0.069 & 0.995 & 0.806 \\
Fokker--Planck type & 2 & 3.476e-03 & 3.476e-03 & 0.228 & 0.228 & 0.995 & 0.453 \\
Fokker--Planck type & 4 & -- & -- & -- & -- & -- & -- \\
Implicit interaction & 2 & 1.312e-03 & 2.434e-03 & 0.537 & 0.536 & 0.977 & 0.092 \\
\bottomrule
\end{tabular}


==> generated/experiment_protocol_table.tex <==
\begin{tabular}{@{}lclccccc@{}}
\toprule
Experiment & $d$ & domain & $\tau$ & steps & requested $T=N\tau$ & widths $(T,q,\rho)$ & base $N$ \\
\midrule
Small-$\tau$ pair & 1 & $[-1,1]$ & 0.00125--0.02 & 1 & -- & 32,64,-- & 2400 \\
Pointwise PDE diagnostic & 1 & $[-1,1]$ & 0.000625--0.02 & 1 & -- & 64,64,64 & 3000 \\
Pair recovery & 1 & -- & -- & -- & -- & -- & -- \\
Finite-grid certificate & 1 & $[-0.6,0.6]$ & 0.020 & 1 & 0.020 & varied,64,-- & 2400 \\
Entropy--potential & 1 & $[-1,1]$ & 2.500e-03 & 1000 & 2.500 & 64,64,64 & 250 \\
Entropy--potential & 2 & $[-1,1]^2$ & 2.500e-03 & 480 & 1.200 & 64,64,64 & 250 \\
$\HK$ entropy & 2 & -- & -- & -- & -- & -- & -- \\
$\HK$ entropy & 8 & $[-3.5,3.5]^8$ & 6.250e-04 & 240 & 0.150 & 64,64,64 & 250 \\
Fokker--Planck & 2 & $[-5,5]^2$ & 1.250e-03 & 960 & 1.200 & 64,64,64 & 250 \\
Fokker--Planck & 4 & -- & -- & -- & -- & -- & -- \\
Coercive interaction & 2 & $[-1,1]^2$ & 2.500e-03 & 120 & 0.300 & 256,256,256 & 400 \\
Pair restriction & 1 & $[-1,1]$ & 2.500e-03 & 320 & 0.800 & 64,64,64 & 250 \\
Optimization budget & 2 & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}


==> generated/interaction_results.tex <==
On residual measurement grids $128^2$ and $512^2$, the implicit residual is $0.0207$ and $0.0665$, respectively. Strong-form consistency remains spatially unresolved. These measurements do not certify a continuum error bound.


==> generated/run_provenance.tex <==
The retained results use their archived per-case numerical sources, including the entropy 8D recovery repair. The pointwise PDE diagnostic comes from a separate completed MPS run; its fixed trained weights are evaluated in CPU float64 for spatial differentiation. Source hashes are retained with each result.


==> sections/experiment_setup.tex <==
% Load once in your preamble, after your existing package declarations.
% Existing definitions are retained; no theorem numbering or layout is changed.
\ifdefined\HKExperimentSetupLoaded\else
\let\HKExperimentSetupLoaded\empty
\RequirePackage{amsmath,amssymb,graphicx,array,booktabs,float,placeins,caption}
\providecommand{\HK}{\mathsf{H\kern-3pt K}}
\providecommand{\safeinput}[1]{\input{#1}}
\providecommand{\safeincludegraphics}[2][]{\includegraphics[#1]{#2}}
\ifdefined\selectedtable\else
\RequirePackage{catchfile}
\ExplSyntaxOn
\tl_new:N \l_hk_selected_source_tl
\tl_new:N \l_hk_selected_prefix_tl
\tl_new:N \l_hk_selected_body_tl
\tl_new:N \l_hk_selected_suffix_tl
\tl_new:N \l_hk_selected_row_tl
\tl_new:N \l_hk_selected_output_tl
\seq_new:N \l_hk_selected_parts_seq
\seq_new:N \l_hk_selected_rows_seq
\seq_new:N \l_hk_selected_indices_seq
\int_new:N \l_hk_selected_columns_int
\int_new:N \l_hk_selected_row_int
\msg_new:nnn { hk-selected-table } { invalid }
  { Invalid~selected~table:~#1. }
\cs_generate_variant:Nn \seq_set_split:Nnn { NnV }
\cs_generate_variant:Nn \seq_if_in:NnTF { NV }
\cs_generate_variant:Nn \regex_match:nnTF { nV }

\cs_new_protected:Npn \hk_selected_fail:n #1
  { \msg_fatal:nnn { hk-selected-table } { invalid } {#1} }
\cs_new_protected:Npn \hk_selected_require_two:n #1
  {
    \int_compare:nNnF { \seq_count:N \l_hk_selected_parts_seq } = {2}
      { \hk_selected_fail:n { expected~exactly~one~#1 } }
  }
\cs_new_protected:Npn \selectedtable #1#2
  {
    \group_begin:
    \file_if_exist:nF {#1}
      { \hk_selected_fail:n { missing~file~\tl_to_str:n {#1} } }
    \regex_match:nnTF { \A \s* [1-9][0-9]* ( \s*,\s* [1-9][0-9]* )* \s* \Z } {#2}
      { }
      { \hk_selected_fail:n { expected~a~nonempty~comma-separated~list~of~positive~integers } }
    \seq_clear:N \l_hk_selected_indices_seq
    \clist_map_inline:nn {#2}
      {
        \tl_set:Nn \l_hk_selected_row_tl {##1}
        \tl_trim_spaces:N \l_hk_selected_row_tl
        \regex_match:nVTF { \A [1-9][0-9]* \Z } \l_hk_selected_row_tl
          { }
          { \hk_selected_fail:n { row~indices~must~be~positive~integers } }
        \seq_if_in:NVTF \l_hk_selected_indices_seq \l_hk_selected_row_tl
          { \hk_selected_fail:n { duplicate~row~index } }
          { \seq_put_right:NV \l_hk_selected_indices_seq \l_hk_selected_row_tl }
      }
    \seq_if_empty:NT \l_hk_selected_indices_seq
      { \hk_selected_fail:n { empty~row~selection } }
    \CatchFileDef\l_hk_selected_source_tl{#1}{\endlinechar=32\relax}
    \seq_set_split:NnV \l_hk_selected_parts_seq {\midrule} \l_hk_selected_source_tl
    \hk_selected_require_two:n { midrule }
    \seq_pop_left:NN \l_hk_selected_parts_seq \l_hk_selected_prefix_tl
    \seq_pop_left:NN \l_hk_selected_parts_seq \l_hk_selected_body_tl
    \seq_set_split:NnV \l_hk_selected_parts_seq {\bottomrule} \l_hk_selected_body_tl
    \hk_selected_require_two:n { bottomrule }
    \seq_pop_left:NN \l_hk_selected_parts_seq \l_hk_selected_body_tl
    \seq_pop_left:NN \l_hk_selected_parts_seq \l_hk_selected_suffix_tl
    \tl_trim_spaces:N \l_hk_selected_suffix_tl
    \tl_if_eq:NnF \l_hk_selected_suffix_tl {\end{tabular}}
      { \hk_selected_fail:n { malformed~tabular~footer } }
    \regex_match:nVTF { \A \s* \c{begin} \{ tabular \} } \l_hk_selected_prefix_tl
      { }
      { \hk_selected_fail:n { malformed~tabular~opening } }
    \seq_set_split:NnV \l_hk_selected_parts_seq {\toprule} \l_hk_selected_prefix_tl
    \hk_selected_require_two:n { toprule }
    \seq_set_split:NnV \l_hk_selected_parts_seq {\\} \l_hk_selected_prefix_tl
    \hk_selected_require_two:n { header~row }
    \seq_pop_right:NN \l_hk_selected_parts_seq \l_hk_selected_row_tl
    \tl_trim_spaces:N \l_hk_selected_row_tl
    \tl_if_empty:NF \l_hk_selected_row_tl
      { \hk_selected_fail:n { malformed~header~row~terminator } }
    \seq_set_split:NnV \l_hk_selected_parts_seq {&} \l_hk_selected_prefix_tl
    \int_set:Nn \l_hk_selected_columns_int { \seq_count:N \l_hk_selected_parts_seq }
    \int_compare:nNnF {\l_hk_selected_columns_int} > {1}
      { \hk_selected_fail:n { missing~table~columns } }
    \seq_set_split:NnV \l_hk_selected_rows_seq {\\} \l_hk_selected_body_tl
    \seq_pop_right:NN \l_hk_selected_rows_seq \l_hk_selected_row_tl
    \tl_trim_spaces:N \l_hk_selected_row_tl
    \tl_if_empty:NF \l_hk_selected_row_tl
      { \hk_selected_fail:n { malformed~data~row~terminator } }
    \seq_map_inline:Nn \l_hk_selected_indices_seq
      {
        \int_compare:nNnT {##1} > {\seq_count:N \l_hk_selected_rows_seq}
          { \hk_selected_fail:n { row~index~out~of~range } }
      }
    \tl_set_eq:NN \l_hk_selected_output_tl \l_hk_selected_prefix_tl
    \tl_put_right:Nn \l_hk_selected_output_tl {\midrule}
    \int_zero:N \l_hk_selected_row_int
    \seq_map_inline:Nn \l_hk_selected_rows_seq
      {
        \int_incr:N \l_hk_selected_row_int
        \seq_set_split:Nnn \l_hk_selected_parts_seq {&} {##1}
        \int_compare:nNnF {\seq_count:N \l_hk_selected_parts_seq} = {\l_hk_selected_columns_int}
          { \hk_selected_fail:n { inconsistent~column~count } }
        \tl_set:Nx \l_hk_selected_row_tl {\int_use:N \l_hk_selected_row_int}
        \seq_if_in:NVTF \l_hk_selected_indices_seq \l_hk_selected_row_tl
          { \tl_put_right:Nn \l_hk_selected_output_tl {##1\\} }
          { }
      }
    \tl_put_right:Nn \l_hk_selected_output_tl {\bottomrule}
    \tl_put_right:NV \l_hk_selected_output_tl \l_hk_selected_suffix_tl
    \tl_use:N \l_hk_selected_output_tl
    \group_end:
  }
\ExplSyntaxOff
\fi
\fi

